AP-BSN: Self-Supervised Denoising for Real-World Images via Asymmetric PD and Blind-Spot Network

Blind-spot network (BSN) and its variants have made significant advances in self-supervised denoising. Nevertheless, they are still bound to synthetic noisy inputs due to less practical assumptions like pixel-wise independent noise. Hence, it is challenging to deal with spatially correlated real-world noise using self-supervised BSN. Recently, pixel-shuffle downsampling (PD) has been proposed to remove the spatial correlation of real-world noise. However, it is not trivial to integrate PD and BSN directly, which prevents the fully self-supervised denoising model on real-world images. We propose an Asymmetric PD (AP) to address this issue, which introduces different PD stride factors for training and inference. We systematically demonstrate that the proposed AP can resolve inherent trade-offs caused by specific PD stride factors and make BSN applicable to practical scenarios. To this end, we develop AP-BSN, a state-of-the-art self-supervised denoising method for real-world sRGB images. We further propose random-replacing refinement, which significantly improves the performance of our AP-BSN without any additional parameters. Extensive studies demonstrate that our method outperforms the other self-supervised and even unpaired denoising methods by a large margin, without using any additional knowledge, e.g., noise level, regarding the underlying unknown noise.

==> main/figs/fig_clean_self.tex <==
\begin{figure}[t!]
    \renewcommand{\wp}{0.495\linewidth}
    \captionsetup[subfloat]{font=normalsize}
    \centering
    \subfloat[Clean]
    {\includegraphics[width=\wp]{example-image-a}}
    \hfill
    \subfloat[$\text{AP}_{55}$]
    {\includegraphics[width=\wp]{example-image-a}}
    \\
    \subfloat[$\text{AP}_{22}$]
    {\includegraphics[width=\wp]{example-image-a}}
    \hfill
    \subfloat[$\text{AP}_{52}$]
    {\includegraphics[width=\wp]{_src/main/pdsf/0278_N_z.png}\label{fig:prb_pdbsn_bsnpd5_2}}
    \\
    \vspace{-2mm}
    \caption{
        \textbf{Issues on using blind-spot network (BSN) with PD for real-world noisy images.}
        %
        (a), (b) Real-world noisy and clean image from the SIDD dataset.
        %
        % (b) Directly training BSN to real-world images and denoising result of (a).
        %
        % (c) Training BSN and denoising (a) using Pixel-shuffle Down-sampling (PD) with stride factor 5.
        (c), (d) Training BSN and inference using PD with stride factor 2, 5 repectively.
        %
        Simply integrating BSN and PD suffers from remaining noise or destructed image texture.
        %
        (e) Results of Zhou~\etal\cite{whenAWGN} which utilize pre-trained AWGN denoiser and PD.
        %
        (f) Our \proposed{} reconstruct clean texture without any artifacts.
    }
    \label{fig:pd_stride_factor}
    \vspace{-4mm}
\end{figure}

==> main/figs/tab_ablation_backup.tex <==
\begin{table}[t]
    \centering
    %\renewcommand{\arraystretch}{0.9}
    \newcommand{\psnrnssim}[2]{\makecell{\small{#1} / \small{#2}}}
    \definecolor{Gray}{gray}{0.90}
    \begin{tabularx}{1.0\linewidth}{cc | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X}
        \toprule
        \multirow{3}{*}{\makecell{\textbf{Training} \\ \small{noise type}}} & 
        \multirow{3}{*}{\makecell{\textbf{Training} \\ \small{stride factor}}} &
        \multicolumn{2}{c}{\makecell{\textbf{Inference} \\ \small{noise type}}} \\
        &&
        \makecell{Synthetic \\ \small{($\sigma = 25$)}} & 
        \makecell{Real} \\
        \midrule
        % \multirow{3}{*}{Synthetic} & 3   & \psnrnssim{36.29}{0.841} & \psnrnssim{32.95}{0.740} \\
        %                                     & 4   & \psnrnssim{36.20}{0.836} & \psnrnssim{33.35}{0.771} \\
        %                                     & 5   & \psnrnssim{36.09}{0.836} & \psnrnssim{33.53}{0.787} \\
        \multirow{3}{*}{\makecell{Synthetic \\ \small{($\sigma \in [0, 50]$)}}} & 3   & \psnrnssim{??.??}{0.???} & \psnrnssim{??.??}{0.???} \\
                                            & 4   & \psnrnssim{??.??}{0.???} & \psnrnssim{??.??}{0.???} \\
                                            & 5   & \psnrnssim{??.??}{0.???} & \psnrnssim{??.??}{0.???} \\
        \midrule
        \multirow{3}{*}{Real}      & 3   & \psnrnssim{29.14}{0.537} & \psnrnssim{33.58}{0.761} \\
                                            & 4   & \psnrnssim{31.56}{0.715} & \psnrnssim{34.48}{0.808} \\
                                            & 5   & \psnrnssim{32.05}{0.768} & \psnrnssim{\textbf{34.86}}{\textbf{0.822}} \\
        \bottomrule
    \end{tabularx}
    \caption{
        \textbf{Comparison between }
    }
    \label{tab:bsn_real_syn}
\end{table}

==> main/figs/tab_bsn-real-syn.tex <==
\begin{table}[t]
    \centering
    %\renewcommand{\arraystretch}{0.9}
    
    \footnotesize
    
    \newcommand{\psnrnssim}[2]{\makecell{\footnotesize{#1} / \footnotesize{#2}}}
    \definecolor{Gray}{gray}{0.90}
    \begin{tabularx}{1.0\linewidth}{cc | >{\centering\arraybackslash}X | >{\centering\arraybackslash}X}
        \toprule
        \multirow{3}{*}{\makecell{\textbf{Training} \\ \small{Noise type}}} & 
        \multirow{3}{*}{\makecell{\textbf{Training} \\ \small{Images}}} &
        \multicolumn{2}{c}{\makecell{\textbf{Inference}  \\ \small{Noise type}}} \\
        && \makecell{AWGN \\ \small{($\sigma = 25$)}} & \makecell{Real} \\
        \midrule
        \multirow{2}{*}{\makecell{AWGN \\ \small{($\sigma \in [0, 50]$)}}} & DIV2K & \psnrnssim{35.47}{0.819} & \psnrnssim{33.40}{0.790} \\
        & SIDD & \psnrnssim{\textbf{35.85}}{\textbf{0.828}} & \psnrnssim{33.17}{0.774} \\
        \midrule
        \multirow{2}{*}{Real} & DND & \psnrnssim{29.41}{0.685} & \psnrnssim{34.48}{0.818} \\
        & SIDD & \psnrnssim{32.05}{0.768} & \psnrnssim{\textbf{34.86}}{\textbf{0.822}} \\
        \bottomrule
    \end{tabularx}
    \caption{
        \textbf{Effect of training noise type and image contents.}
        %
        We train \proposed{} for blind-AWGN on clean images in the SIDD~\cite{SIDD} or DIV2K~\cite{DIV2K} training dataset.
        %
        Also we compared them and another 2 models trained using real-world datatset, \eg, SIDD and DND toward AWGN and real-world denoising.
        %
    }
    \label{tab:bsn_real_syn}
\end{table}

==> main/figs/tab_main_working.tex <==
\begin{table*}[t]
    \centering
    \newcommand{\ts}{\,\,}
    \newcommand{\ourspad}{\:}
    %\newcommand{\ours}{^\dagger}
    % \newcommand{\ours}{{^\textbf{\tiny{O}}}}
    \newcommand{\ours}{{^\diamond}}
    \newcommand{\fromRpad}{\:}
    \newcommand{\fromR}{{^\textbf{\tiny{R}}}}
    \newcommand{\selfen}{^*}
    \newcommand{\benchmark}{\dagger}
    
    \small
    
    \begin{tabularx}{\linewidth}{cc >{\raggedright\arraybackslash}X  ccccccc}
        \toprule
        && \multirow{2}{*}{Method} & \multirow{2}{*}{Params} && \multicolumn{2}{c}{SIDD} && \multicolumn{2}{c}{DND} \\
        && & && PSNR$^\uparrow$(dB) & SSIM$^\uparrow$ && PSNR$^\uparrow$(dB) & SSIM$^\uparrow$  \\
        \midrule
        
        \multirow{2}{*}{\makecell{Non-learning based}} 
        && BM3D~\cite{BM3D} & - && 25.65 & 0.685 && 34.51 & 0.851 \\
        && WNNM~\cite{WNNM} & - && 25.78 & 0.809 && 34.67 & 0.865 \\
        \midrule
        
        \multirow{3}{*}{\makecell{Supervised \\ (Synthetic pairs)}}
        && DnCNN~\cite{DnCNN} & 0.67M && 23.66 & 0.583 && 32.43 & 0.790 \\
        && CBDNet~\cite{CBDNet} & && 33.28 & 0.868 && 38.05 & 0.942 \\
        && Zhou~\etal~\cite{whenAWGN} & && $\ourspad$ \text{34.00}$\ours$ & $\ourspad$ \text{0.898}$\ours$ && 38.40 & 0.945 \\
        \midrule
        
        \multirow{4}{*}{\makecell{Supervised \\ (Real pairs)}} 
        && DnCNN~\cite{DnCNN} & && $\ourspad$ \text{35.13}$\ours$ & $\ourspad$ \text{0.896}$\ours$ && $\ourspad$ \text{37.89}$\ours$ & $\ourspad$ \text{0.932}$\ours$ \\
        && AINDNet (R)$\selfen$~\cite{AINDNet} & && 38.84 & 0.951 && 39.34 & 0.952 \\
        && VDN~\cite{VDN} & && 39.26 & 0.955 && 39.38 & 0.952 \\
        && DANet\cite{DANet} & && 39.43 & 0.956 && 39.58 & 0.955 \\
        % && DIDN~\cite{DIDN} & && 39.82 & 0.973 && - & - & \\
        \midrule
        
        \multirow{3}{*}{\makecell{Unsupervised \\ (Unpaired)}}
        && GCBD~\cite{GCBD} & && - & - && 35.58 & 0.922 \\
        && C2N~\cite{C2N} $+$ DIDN$\selfen$~\cite{DIDN} & && 35.35 & 0.937 && 37.28 & 0.924 \\
        && D-BSN~\cite{DBSN} $+$ MWCNN~\cite{MWCNN} & && - & - && 37.93 & 0.937 \\
        \midrule
        
        \multirow{7}{*}{\makecell{Self-supervised}}
        && Noise2Void~\cite{Noise2Void} & && $\fromRpad$ \text{27.68}$\fromR$ & $\fromRpad$ \text{0.668}$\fromR$ && - & - \\
        && Noise2Self~\cite{Noise2Self} & && $\fromRpad$ \text{29.56}$\fromR$ & $\fromRpad$ \text{0.808}$\fromR$ && - & - \\
        % && Laine~\etal~\cite{Laine2019} & $\ts$ ??.??$^+$ & $\ts$ 0.???$^+$ && $\ts$ ??.??$^+$ & $\ts$ 0.???$^+$ & \\
        && Noisy-As-Clean~\cite{NAC} & 0.78M && - & - && 36.20 & 0.925 \\
        % && NN $+$ BM3D~\cite{zheng2020unsupervised} & 33.18 & 0.895 && 37.10 & 0.944 & \\
        && R2R~\cite{R2R} & 0.67M && 34.78 & 0.898 && - & - \\
        && \textbf{\proposed{} (Ours)} & 3.7M && \textbf{34.90} & \textbf{0.900} && \textbf{37.46} & \textbf{0.924} \\
        %&& \textbf{R-BSN$^{\times 4}$} (Ours) & \textbf{35.78} & \textbf{0.925} && \textbf{??.??} & \textbf{0.???} & \\
        && \textbf{\proposed{}$\:\:$ $+$ $\rrpp$ (Ours)} & 3.7M && \textbf{35.97} & \textbf{0.925} && \textbf{38.09} & \textbf{0.937} \\
        && \textbf{\proposed{}$^\benchmark$ $+$ $\rrpp$ (Ours)} & 3.7M && \textbf{36.91} & \textbf{0.931} && - & - \\
        \bottomrule
    \end{tabularx}
    \vspace{-2mm}
    \caption{
        \textbf{Quantitative comparison of various denoising methods on the SIDD and DND benchmarks.}
        %
        We note that several supervised methods leverage SIDD noisy-clean pairs for training and perform much better than our AP-BSN, while we use noisy sRGB images only for training.
        %
        By default, we report official evaluation results from SIDD and DND benchmark websites.
        %
        $\diamond$ and \textbf{R} indicate that the performances are evaluated by ourselves, or reported from R2R~\cite{R2R}, respectively.
        %
        We also mark methods with $\ast$ which adopt self-ensemble strategy~\cite{EDSR}.
        %
        $\benchmark$ denotes that the model is trained on SIDD benchmark images in a fully self-supervised fashion.
    }
    \label{tab:main}
    \vspace{-4mm}
\end{table*}

==> main/figs/tab_pdsf.tex <==
\begin{table}[t]
    \centering
    %\renewcommand{\arraystretch}{0.9}
    \definecolor{Gray}{gray}{0.95}
    \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X >{\centering\arraybackslash}X | cc}
        \toprule
        %\makecell{w/o RPR \\ \footnotesize{PSNR (dB)}}
        \makecell{\textbf{Training} \\ \small{stride factor}} & \makecell{\textbf{Inference} \\ \small{stride factor}} & PSNR$^\uparrow$(dB) & SSIM$^\uparrow$ \\
        \midrule
        w/o \small{PD} & w/o \small{PD}             & 23.72 & 0.328 \\
        %2              & 2                          & 25.79 & 0.412 \\
        % 4              & 4                          & 33.66 & 0.763 \\
        %5              & 5                          & 33.38 & 0.761 \\
        \midrule
        2                   & \cellcolor{Gray}    & 25.79 & 0.412 \\
        3                   & \cellcolor{Gray}    & 33.58 & 0.761 \\
        4                   & \cellcolor{Gray}    & 34.48 & 0.808 \\
        \textbf{5}          & \cellcolor{Gray}    & \textbf{34.86} & \textbf{0.822} \\
        6                   & \multirow{-5}{*}{\cellcolor{Gray}\large{\textbf{2}}} & 34.45 & 0.809 \\
        \midrule
        \cellcolor{Gray}    & w/o \small{PD}        & 30.92 & 0.714 \\
        \cellcolor{Gray}    & \textbf{2}            & \textbf{34.86} & \textbf{0.822} \\
        \cellcolor{Gray}    & 3                     & 34.43 & 0.794 \\
        \cellcolor{Gray}    & 4                     & 33.82 & 0.766 \\
        \multirow{-5}{*}{\cellcolor{Gray}\large{\textbf{5}}}    & 5                     & 33.38 & 0.761 \\
        % \midrule
        % \rowcolor{Gray}
        % \textbf{5} & \textbf{2} & \textbf{34.86} & \textbf{0.822} \\
        \bottomrule
    \end{tabularx}
    \caption{
        \textbf{Experiments on Asymmetric PD with diverse stride factor.}
        %
        First row box
    }
    \label{tab:pd_stride_factor}
\end{table}

==> supple/figs/fig_network.tex <==
\begin{figure*}[t!]
    \renewcommand{\wp}{1.0\linewidth}
    \centering
    \includegraphics[width=\wp]{_src/supple/network/network.pdf}
    % \includegraphics[width=\wp, height=0.4\linewidth]{example-image-a}
    \\
    \vspace{-2mm}
    \caption{
        \textbf{Visualization of BSN architecture in our \proposed{}.}
        %
        We modify the network D-BSN from Wu~\etal~\cite{DBSN} into the network have more layer channel, basic modules.
        %
        Also instead of using Multiple Dialted Convolution (MDC) module, our BSN utilizes Dilated Convolution (DC) module which has single branch of dilated convolution layer.
        %
        More details about D-BSN are available in Wu~\etal~\cite{DBSN}.
    }
    \label{fig:network}
    \vspace{-4mm}
\end{figure*}

==> supple/figs/tab_network.tex <==
\begin{table}[t]
    \centering
    %\renewcommand{\arraystretch}{0.9}
    \definecolor{Gray}{gray}{0.95}
    \begin{tabularx}{\linewidth}{cc >{\centering\arraybackslash}X >{\centering\arraybackslash}X | cc}
        \toprule
        %\makecell{w/o RPR \\ \footnotesize{PSNR (dB)}}
        \makecell{BSN} & \makecell{layer \\ channel} & module & params & PSNR$^\uparrow$(dB) \\
        \midrule
        \makecell{modified \\ (used)} & 128 & 9 DC & 3.7M & ??.?? \\
        D-BSN & 96 & 6 MDC & 4.0M & ??.?? \\
        \bottomrule
    \end{tabularx}
    \caption{
        \textbf{Ablation study on BSN architecture on SIDD validation dataset.}
        %
        First row box
    }
    \label{tab:network}
\end{table}
